Prospects for Improved Understanding of Isotopic Reactor Antineutrino Fluxes

Predictions of antineutrino fluxes produced by fission isotopes in a nuclear reactor have recently received increased scrutiny due to observed differences in predicted and measured inverse beta decay (IBD) yields, referred to as the 'reactor antineutrino flux anomaly.' In this paper, global fits are applied to existing IBD yield measurements to produce constraints on antineutrino production by individual plutonium and uranium fission isotopes. We find that fits including measurements from highly 235U-enriched cores and fits including Daya Bay's new fuel evolution result produce discrepant best-fit IBD yields for 235U and 239Pu. This discrepancy can be alleviated in a global analysis of all datasets through simultaneous fitting of 239Pu, 235U, and 238U yields. The measured IBD yield of U238 in this analysis is (7.02 +/- 1.65) x 10^-43 cm2/fission, nearly two standard deviations below existing predictions. Future hypothetical IBD yield measurements by short-baseline reactor experiments are examined to determine their possible impact on global understanding of isotopic IBD yields. It is found that future improved short-baseline IBD yield measurements at both high-enriched and low-enriched cores can significantly improve constraints for 235U, 238U, and 239Pu, providing comparable or superior precision to existing conversion- and summation-based antineutrino flux predictions. Systematic and experimental requirements for these future measurements are also investigated.

==> author.tex <==
%%% Generation information for this file
%%% Wed Jun 29 08:55:36 2016
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList/FuelEvolution2016
%%% ../AuthGen.py dyb_collabotion_list_20150803.xls 20150803 
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706, USA}}
\newcommand{\Yale}{\affiliation{Department~of~Physics, Yale~University, New~Haven, Connecticut 06520, USA}}
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973, USA}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125, USA}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211, USA}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616, USA}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720, USA}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801, USA}}
\newcommand{\RPI}{\affiliation{Department~of~Physics, Applied~Physics, and~Astronomy, Rensselaer~Polytechnic~Institute, Troy, New~York  12180, USA}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187, USA}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544, USA}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061, USA}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221, USA}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720, USA}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas  77204, USA}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague, Czech~Republic}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122, USA}}
\newcommand{\CUC}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago, Chile}} % update 20140911 use r23215 for Spanish
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group}}% updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011, USA}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453, USA}} % add 20160311 for Sunej's 'now at'
%\newcommand{\BCC}{\affiliation{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453, USA}} % add 20160311 for Sunej's 'now at'
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU\NUU
\author{D.~Cao}\NJU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{Y.~L.~Chan}\CUHK
\author{J.~F.~Chang}\IHEP
\author{L.~C.~Chang}\NCTU
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{Q.~Y.~Chen}\SDU
\author{S.~M.~Chen}\TsingHua
\author{Y.~X.~Chen}\NCEPU
\author{Y.~Chen}\SZU
\author{J.-H.~Cheng}\NCTU
\author{J.~Cheng}\SDU
\author{Y.~P.~Cheng}\IHEP
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{A.~Chukanov}\Dubna
\author{J.~P.~Cummings}\Siena
\author{Z.~Y.~Deng}\IHEP
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{M.~Dolgareva}\Dubna
\author{J.~Dove}\UIUC
\author{D.~A.~Dwyer}\LBNL
\author{W.~R.~Edwards}\LBNL
\author{R.~Gill}\BNL
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{M.~Grassi}\IHEP
\author{W.~Q.~Gu}\SJTU
\author{M.~Y.~Guan}\IHEP
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{Z.~Guo}\TsingHua
\author{R.~W.~Hackenburg}\BNL
\author{R.~Han}\NCEPU
\author{S.~Hans}\BCC\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{A.~Higuera}\UH
\author{Y.~K.~Hor}\VirginiaTech
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{T.~Hu}\IHEP
\author{W.~Hu}\IHEP
\author{E.~C.~Huang}\UIUC
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{P.~Huber}\VirginiaTech
\author{W.~Huo}\USTC
\author{G.~Hussain}\TsingHua
\author{D.~E.~Jaffe}\BNL
\author{P.~Jaffke}\VirginiaTech
\author{K.~L.~Jen}\NCTU
\author{S.~Jetter}\IHEP
\author{X.~P.~Ji}\NanKai\TsingHua
\author{X.~L.~Ji}\IHEP
\author{J.~B.~Jiao}\SDU
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{J.~Joshi}\BNL
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{K.~K.~Kwan}\CUHK
\author{M.~W.~Kwok}\CUHK
\author{T.~Kwok}\HKU
\author{T.~J.~Langford}\Yale
\author{K.~Lau}\UH
\author{L.~Lebanowski}\TsingHua
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{C.~Li}\SDU
\author{D.~J.~Li}\USTC
\author{F.~Li}\IHEP
\author{G.~S.~Li}\SJTU
\author{Q.~J.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\HKU\VirginiaTech
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{S.~K.~Lin}\UH
\author{Y.-C.~Lin}\NTU
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{D.~W.~Liu}\UH
\author{J.~L.~Liu}\SJTU
\author{J.~C.~Liu}\IHEP
\author{C.~W.~Loh}\NJU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{J.~S.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{Z.~Lv}\XJTU
\author{Q.~M.~Ma}\IHEP
\author{X.~Y.~Ma}\IHEP
\author{X.~B.~Ma}\NCEPU
\author{Y.~Q.~Ma}\IHEP
\author{Y.~Malyshkin}\CUC
\author{D.~A.~Martinez Caicedo}\IIT
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{I.~Mitchell}\UH
\author{M.~Mooney}\BNL
\author{Y.~Nakajima}\LBNL
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{H.~Y.~Ngai}\HKU
\author{A.~T.~Nguyen}\NCTU
\author{Z.~Ning}\IHEP
\author{J.~P.~Ochoa-Ricoux}\CUC
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{V.~Pec}\Charles
\author{J.~C.~Peng}\UIUC
\author{L.~Pinsky}\UH
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\RPI
\author{J.~Ren}\CIAE
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\Charles
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{G.~X.~Sun}\IHEP
\author{J.~L.~Sun}\CGNPG
\author{W.~Tang}\BNL
\author{D.~Taychenachev}\Dubna
\author{K.~Treskov}\Dubna
\author{K.~V.~Tsang}\LBNL
\author{C.~E.~Tull}\LBNL
\author{N.~Viaux}\CUC
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\WM\ZSU
\author{X.~Wang}\NUDT
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~Wang}\IHEP
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\TsingHua
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{L.~Whitehead}\UH
\author{T.~Wise}\Wisconsin
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{S.~C.~F.~Wong}\ZSU
\author{E.~Worcester}\BNL
\author{C.-H.~Wu}\NCTU
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU
\author{J.~K.~Xia}\IHEP
\author{Z.~Z.~Xing}\IHEP
\author{J.~Y.~Xu}\CUHK
\author{J.~L.~Xu}\IHEP
\author{Y.~Xu}\ZSU
\author{T.~Xue}\TsingHua
\author{C.~G.~Yang}\IHEP
\author{H.~Yang}\NJU
\author{L.~Yang}\DGUT
\author{M.~S.~Yang}\IHEP
\author{M.~T.~Yang}\SDU
\author{M.~Ye}\IHEP
\author{Z.~Ye}\UH
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{Z.~Y.~Yu}\IHEP
\author{S.~Zeng}\IHEP
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\TsingHua
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~M.~Zhang}\ZSU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~Y.~Zhang}\IHEP
\author{Z.~P.~Zhang}\USTC
\author{J.~Zhao}\IHEP
\author{Y.~B.~Zhao}\IHEP
\author{W.~L.~Zhong}\IHEP
\author{L.~Zhou}\IHEP
\author{N.~Zhou}\USTC
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP


==> author_2014.tex <==
%%% Generation information for this file
%%% 20140529 09:01:16
%%% /Users/djaffe/Documents/Reactor/work/r22373/NuWa-trunk/dybgaudi/Documentation/AuthorList/Reactor2015PRL
%%% ../AuthGen.py dybCollaborationList_20140301.xls 20140301 
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin, USA}}
\newcommand{\Yale}{\affiliation{Department~of~Physics, Yale~University, New~Haven, Connecticut, USA}}
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York, USA}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California, USA}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York, USA}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois, USA}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California, USA}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois, USA}}
\newcommand{\RPI}{\affiliation{Department~of~Physics, Applied~Physics, and~Astronomy, Rensselaer~Polytechnic~Institute, Troy, New~York, USA}}
\newcommand{\SJTU}{\affiliation{Shanghai~Jiao~Tong~University, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia, USA}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey, USA}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia, USA}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio, USA}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California, USA}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas, USA}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague}}
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania, USA}}
\newcommand{\CUC}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago, Chile}} % update 20140911 use r23215 for Spanish
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group}}% updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa, USA}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU\NUU
\author{I.~Butorov}\Dubna
\author{D.~Cao}\NJU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{W.~R.~Cen}\IHEP
\author{Y.~L.~Chan}\CUHK
\author{J.~F.~Chang}\IHEP
\author{L.~C.~Chang}\NCTU
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{Q.~Y.~Chen}\SDU
\author{S.~M.~Chen}\TsingHua
\author{Y.~X.~Chen}\NCEPU
\author{Y.~Chen}\SZU
\author{C.-H.~Cheng}\NCTU
\author{J.~Cheng}\SDU
\author{Y.~P.~Cheng}\IHEP
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{J.~P.~Cummings}\Siena
\author{J.~de Arcos}\IIT
\author{Z.~Y.~Deng}\IHEP
\author{X.~Ding}\IHEP
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{E.~Draeger}\IIT
\author{D.~A.~Dwyer}\LBNL
\author{W.~R.~Edwards}\LBNL
\author{S.~R.~Ely}\UIUC
\author{R.~Gill}\BNL
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{M.~Grassi}\IHEP
\author{W.~Q.~Gu}\SJTU
\author{M.~Y.~Guan}\IHEP
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{R.~W.~Hackenburg}\BNL
\author{R.~Han}\NCEPU
\author{S.~Hans}\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{Y.~K.~Hor}\VirginiaTech
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{L.~M.~Hu}\BNL
\author{L.~J.~Hu}\BNU
\author{T.~Hu}\IHEP
\author{W.~Hu}\IHEP
\author{E.~C.~Huang}\UIUC
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{P.~Huber}\VirginiaTech
\author{G.~Hussain}\TsingHua
\author{D.~E.~Jaffe}\BNL
\author{P.~Jaffke}\VirginiaTech
\author{K.~L.~Jen}\NCTU
\author{S.~Jetter}\IHEP
\author{X.~P.~Ji}\NanKai\TsingHua
\author{X.~L.~Ji}\IHEP
\author{J.~B.~Jiao}\SDU
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{M.~Kramer}\LBNL\UCB
\author{K.~K.~Kwan}\CUHK
\author{M.~W.~Kwok}\CUHK
\author{T.~Kwok}\HKU
\author{T.~J.~Langford}\Yale
\author{K.~Lau}\UH
\author{L.~Lebanowski}\TsingHua
\author{J.~Lee}\LBNL
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{A.~Leung}\HKU
\author{J.~K.~C.~Leung}\HKU
\author{C.~A.~Lewis}\Wisconsin
\author{D.~J.~Li}\USTC
\author{F.~Li}\IHEP
\author{G.~S.~Li}\SJTU
\author{Q.~J.~Li}\IHEP
\author{S.~C.~Li}\HKU
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{X.~Q.~Li}\NanKai
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{P.~Y.~Lin}\NCTU
\author{S.~K.~Lin}\UH
\author{J.~J.~Ling}\BNL\UIUC
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\UC\IIT
\author{D.~W.~Liu}\UH
\author{H.~Liu}\UH
\author{J.~L.~Liu}\SJTU
\author{J.~C.~Liu}\IHEP
\author{S.~S.~Liu}\HKU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{Q.~M.~Ma}\IHEP
\author{X.~Y.~Ma}\IHEP
\author{X.~B.~Ma}\NCEPU
\author{Y.~Q.~Ma}\IHEP
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{Y.~Meng}\VirginiaTech
\author{I.~Mitchell}\UH
\author{J.~Monari Kebwaro}\XJTU
\author{Y.~Nakajima}\LBNL
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{I.~Nemchenok}\Dubna
\author{H.~Y.~Ngai}\HKU
\author{Z.~Ning}\IHEP
\author{J.~P.~Ochoa-Ricoux}\CUC
\author{A.~Olshevski}\Dubna
\author{H.-R.~Pan}\NTU
\author{S.~Patton}\LBNL
\author{V.~Pec}\Charles
\author{J.~C.~Peng}\UIUC
\author{L.~E.~Piilonen}\VirginiaTech
\author{L.~Pinsky}\UH
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\RPI
\author{B.~Ren}\DGUT
\author{J.~Ren}\CIAE
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\Charles
\author{X.~C.~Ruan}\CIAE
\author{B.~B.~Shao}\TsingHua
\author{H.~Steiner}\UCB\LBNL
\author{G.~X.~Sun}\IHEP
\author{J.~L.~Sun}\CGNPG
\author{W.~Tang}\BNL
\author{K.~V.~Tsang}\LBNL
\author{C.~E.~Tull}\LBNL
\author{Y.~C.~Tung}\NTU
\author{N.~Viaux}\CUC
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\ZSU
\author{W.~W.~Wang}\NJU
\author{X.~Wang}\NUDT
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~Wang}\IHEP
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\TsingHua
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{L.~Whitehead}\UH
\author{T.~Wise}\Wisconsin
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{S.~C.~F.~Wong}\CUHK
\author{E.~Worcester}\BNL
\author{Q.~Wu}\SDU
\author{D.~M.~Xia}\IHEP
\author{J.~K.~Xia}\IHEP
\author{X.~Xia}\SDU
\author{Z.~Z.~Xing}\IHEP
\author{J.~Y.~Xu}\CUHK
\author{J.~L.~Xu}\IHEP
\author{J.~Xu}\BNU
\author{Y.~Xu}\NanKai
\author{T.~Xue}\TsingHua
\author{J.~Yan}\XJTU
\author{C.~G.~Yang}\IHEP
\author{L.~Yang}\DGUT
\author{M.~S.~Yang}\IHEP
\author{M.~T.~Yang}\SDU
\author{M.~Ye}\IHEP
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{G.~Y.~Yu}\NJU
\author{Z.~Y.~Yu}\IHEP
\author{S.~L.~Zang}\NJU
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{Y.~M.~Zhang}\TsingHua
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~M.~Zhang}\ZSU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~Y.~Zhang}\IHEP
\author{Z.~P.~Zhang}\USTC
\author{J.~Zhao}\IHEP
\author{Q.~W.~Zhao}\IHEP
\author{Y.~F.~Zhao}\NCEPU
\author{Y.~B.~Zhao}\IHEP
\author{L.~Zheng}\USTC
\author{W.~L.~Zhong}\IHEP
\author{L.~Zhou}\IHEP
\author{N.~Zhou}\USTC
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP


==> author_may.tex <==
%%% Generation information for this file
%%% Tue May 31 16:29:20 2016
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList/FuelEvolution2016
%%% ../AuthGen.py dyb_collabotion_list_20150803.xls 20150803 
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706, USA}}
\newcommand{\Yale}{\affiliation{Department~of~Physics, Yale~University, New~Haven, Connecticut 06520, USA}}
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973, USA}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125, USA}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211, USA}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616, USA}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720, USA}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801, USA}}
\newcommand{\RPI}{\affiliation{Department~of~Physics, Applied~Physics, and~Astronomy, Rensselaer~Polytechnic~Institute, Troy, New~York  12180, USA}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187, USA}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544, USA}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061, USA}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221, USA}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720, USA}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas  77204, USA}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague, Czech~Republic}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122, USA}}
\newcommand{\CUC}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago, Chile}} % update 20140911 use r23215 for Spanish
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group}}% updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011, USA}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453, USA}} % add 20160311 for Sunej's 'now at'
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU\NUU
\author{D.~Cao}\NJU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{Y.~L.~Chan}\CUHK
\author{J.~F.~Chang}\IHEP
\author{L.~C.~Chang}\NCTU
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{Q.~Y.~Chen}\SDU
\author{S.~M.~Chen}\TsingHua
\author{Y.~X.~Chen}\NCEPU
\author{Y.~Chen}\SZU
\author{J.-H.~Cheng}\NCTU
\author{J.~Cheng}\SDU
\author{Y.~P.~Cheng}\IHEP
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{A.~Chukanov}\Dubna
\author{J.~P.~Cummings}\Siena
\author{Z.~Y.~Deng}\IHEP
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{M.~Dolgareva}\Dubna
\author{J.~Dove}\UIUC
\author{D.~A.~Dwyer}\LBNL
\author{W.~R.~Edwards}\LBNL
\author{R.~Gill}\BNL
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{M.~Grassi}\IHEP
\author{W.~Q.~Gu}\SJTU
\author{M.~Y.~Guan}\IHEP
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{Z.~Guo}\TsingHua
\author{R.~W.~Hackenburg}\BNL
\author{R.~Han}\NCEPU
\author{S.~Hans}\BCC\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{A.~Higuera}\UH
\author{Y.~K.~Hor}\VirginiaTech
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{T.~Hu}\IHEP
\author{W.~Hu}\IHEP
\author{E.~C.~Huang}\UIUC
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{P.~Huber}\VirginiaTech
\author{W.~Huo}\USTC
\author{G.~Hussain}\TsingHua
\author{D.~E.~Jaffe}\BNL
\author{P.~Jaffke}\VirginiaTech
\author{K.~L.~Jen}\NCTU
\author{S.~Jetter}\IHEP
\author{X.~P.~Ji}\NanKai\TsingHua
\author{X.~L.~Ji}\IHEP
\author{J.~B.~Jiao}\SDU
\author{R.~A.~Johnson}\UC
\author{J.~Joshi}\BNL
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{K.~K.~Kwan}\CUHK
\author{M.~W.~Kwok}\CUHK
\author{T.~Kwok}\HKU
\author{T.~J.~Langford}\Yale
\author{K.~Lau}\UH
\author{L.~Lebanowski}\TsingHua
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{C.~Li}\SDU
\author{D.~J.~Li}\USTC
\author{F.~Li}\IHEP
\author{G.~S.~Li}\SJTU
\author{Q.~J.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\HKU\VirginiaTech
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{S.~K.~Lin}\UH
\author{Y.-C.~Lin}\NTU
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{D.~W.~Liu}\UH
\author{J.~L.~Liu}\SJTU
\author{J.~C.~Liu}\IHEP
\author{C.~W.~Loh}\NJU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{J.~S.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{Z.~Lv}\XJTU
\author{Q.~M.~Ma}\IHEP
\author{X.~Y.~Ma}\IHEP
\author{X.~B.~Ma}\NCEPU
\author{Y.~Q.~Ma}\IHEP
\author{Y.~Malyshkin}\CUC
\author{D.~A.~Martinez Caicedo}\IIT
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{I.~Mitchell}\UH
\author{M.~Mooney}\BNL
\author{Y.~Nakajima}\LBNL
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{H.~Y.~Ngai}\HKU
\author{A.~T.~Nguyen}\NCTU
\author{Z.~Ning}\IHEP
\author{J.~P.~Ochoa-Ricoux}\CUC
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{V.~Pec}\Charles
\author{J.~C.~Peng}\UIUC
\author{L.~Pinsky}\UH
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\RPI
\author{J.~Ren}\CIAE
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\Charles
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{G.~X.~Sun}\IHEP
\author{J.~L.~Sun}\CGNPG
\author{W.~Tang}\BNL
\author{D.~Taychenachev}\Dubna
\author{K.~Treskov}\Dubna
\author{K.~V.~Tsang}\LBNL
\author{C.~E.~Tull}\LBNL
\author{N.~Viaux}\CUC
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\WM\ZSU
\author{X.~Wang}\NUDT
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~Wang}\IHEP
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\TsingHua
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{L.~Whitehead}\UH
\author{T.~Wise}\Wisconsin
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{S.~C.~F.~Wong}\ZSU
\author{E.~Worcester}\BNL
\author{C.-H.~Wu}\NCTU
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU\IHEP
\author{J.~K.~Xia}\IHEP
\author{Z.~Z.~Xing}\IHEP
\author{J.~Y.~Xu}\CUHK
\author{J.~L.~Xu}\IHEP
\author{Y.~Xu}\ZSU
\author{T.~Xue}\TsingHua
\author{C.~G.~Yang}\IHEP
\author{H.~Yang}\NJU
\author{L.~Yang}\DGUT
\author{M.~S.~Yang}\IHEP
\author{M.~T.~Yang}\SDU
\author{M.~Ye}\IHEP
\author{Z.~Ye}\UH
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{Z.~Y.~Yu}\IHEP
\author{S.~Zeng}\IHEP
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\TsingHua
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~M.~Zhang}\ZSU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~Y.~Zhang}\IHEP
\author{Z.~P.~Zhang}\USTC
\author{J.~Zhao}\IHEP
\author{Y.~B.~Zhao}\IHEP
\author{W.~L.~Zhong}\IHEP
\author{L.~Zhou}\IHEP
\author{N.~Zhou}\USTC
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP

